TBar: Revisiting Template-based Automated Program Repair

We revisit the performance of template-based APR to build comprehensive knowledge about the effectiveness of fix patterns, and to highlight the importance of complementary steps such as fault localization or donor code retrieval. To that end, we first investigate the literature to collect, summarize and label recurrently-used fix patterns. Based on the investigation, we build TBar, a straightforward APR tool that systematically attempts to apply these fix patterns to program bugs. We thoroughly evaluate TBar on the Defects4J benchmark. In particular, we assess the actual qualitative and quantitative diversity of fix patterns, as well as their effectiveness in yielding plausible or correct patches. Eventually, we find that, assuming a perfect fault localization, TBar correctly/plausibly fixes 74/101 bugs. Replicating a standard and practical pipeline of APR assessment, we demonstrate that TBar correctly fixes 43 bugs from Defects4J, an unprecedented performance in the literature (including all approaches, i.e., template-based, stochastic mutation-based or synthesis-based APR).

==> tables/aprPartPositionP1.tex <==
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
{\bf Bug}   &   \rotatebox[origin=l]{90}{\bf FP1}   &   \rotatebox[origin=l]{90}{\bf FP2}   &   \rotatebox[origin=l]{90}{\bf FP3}   &   \rotatebox[origin=l]{90}{\bf FP4}   &  \rotatebox[origin=l]{90}{\bf FP5}   &   \rotatebox[origin=l]{90}{\bf FP6}   &   \rotatebox[origin=l]{90}{\bf FP7}   &   \rotatebox[origin=l]{90}{\bf FP8}   &   \rotatebox[origin=l]{90}{\bf FP9}   &   \rotatebox[origin=l]{90}{\bf FP10}   &   \rotatebox[origin=l]{90}{\bf FP11}   &   \rotatebox[origin=l]{90}{\bf FP12}   &   \rotatebox[origin=l]{90}{\bf FP13}   &   \rotatebox[origin=l]{90}{\bf FP14}   &   \rotatebox[origin=l]{90}{F\bf P15}                     &   \rotatebox[origin=l]{90}{\bf \# PP\_FP}                     &   \rotatebox[origin=l]{90}{\bf \# CP\_FP}\\
 \hline 
C-1 & & & & & & \ding{174} & & & & & \ding{202} & & \ding{172} & & \ding{172} & 4 & 1\\
C-4 & & \ding{172} \ding{204} \ding{205} & & & & & & & & & & & & & & 3 & 2\\ 
C-7 & & & & \ding{175} & & & & & & & & & $\LEFTcircle^1$ & & & 2 & 1\\ 
C-8 & & & & & & & & & & & & & \ding{202} & & & 1 & 1\\ 
C-9 & & & & & & \ding{204} & & & \ding{109} & & & & & & & 2 & 1\\ 
C-11 & & & & & & & & & & & & & \ding{202} & & & 1 & 1\\  
C-12 & & & & \ding{202} & & & & & & & & & & & & 1 & 1\\ 
C-13 & & & & \ding{175} & & & & & & & & & & & & 1 & 0\\
C-14 & & \ding{202} \ding{203} & & & & & & & & & & & & & & 2 & 2\\
C-16 & & & & & & & & & & & & & & & (\ding{172}) & 1 & 0\\
C-18 & & & & (\ding{172}) & & (\ding{174}) & & & & & (\ding{172}) & & (\ding{172})& & (\ding{202}) & 5 & 1 \\
C-19 & & \ding{206} & & & & & & & & & & & & & & 1 & 1\\
C-20 & & & & & & & & & & \ding{203} & & & & & & 1 & 1\\
C-22 & & & & & & (\ding{174}) & & & & & & & & & (\ding{172}) & 2 & 0\\
C-24 & & & & & & & & & & & & & \ding{202} & & & 1 & 1\\
C-25 & & (\ding{202}) & & & & & & & & & & & (\ding{172}) & & & 2 & 1\\
C-26 & & \ding{172} \ding{203} \ding{204} & & & & & & & & & & & & & & 3 & 2\\
\hline
Cl-2 & & \ding{172} \ding{173} \ding{204} & & & & & & & & & & & & & & 3 & 1\\
Cl-6 & & & & & & (\ding{173}) (\ding{174})& & & & & (\ding{172}) & & (\ding{109}) & & (\ding{202}) & 5 &1  \\
Cl-10& & & & & & & & & & \ding{202}& & & & & & 1& 1\\
Cl-11& & & & & & \ding{173} \ding{174} & & & & & \ding{202} & & \ding{109} & & \ding{202} & 5 &2 \\
Cl-13& & & & & & & & & & & & & & \ding{108}& & 1&1 \\
Cl-18& & & & & & \ding{203} & & & & & \ding{172} & & & & & 2 & 1\\
Cl-19& & & & & &  & & & & & & & & & \ding{172}& 1 & 0\\
Cl-21& & & & & & \ding{172} \ding{174} & & & & & \ding{202} & & \ding{109} & & \ding{172} & 5 & 1\\
Cl-22& & & & & & \ding{172} \ding{174} & & & & & \ding{202} & & \ding{109} & & \ding{172} & 5 & 1\\
Cl-25& & & & & & & & & & & & & \ding{109}& & & 1 & 0 \\
Cl-31& & & & & & \ding{203} & & & & & \ding{172} & & & & & 2& 1\\
Cl-38& & & & & & \ding{172} \ding{173} & & & & & \ding{202} & & & & & 3&1\\
Cl-40& & & & & & & & & \ding{108} & & & & & & & 1 & 1 \\
Cl-46& & & & & & & & & & & & & & & \ding{203}&1 & 1\\
Cl-49& & & & & & (\ding{174}) & & & & & & & & & & 1& 0\\
Cl-59& & & & & & \ding{174}& & & & & & & & & & 1& 0\\
Cl-62& & & & & & \ding{172} \ding{173} \ding{174}& & & & & $\LEFTcircle^1$ & & & & \ding{172}& 5& 1\\
Cl-62& & & & & & \ding{172} \ding{173} \ding{174}& & & & & $\LEFTcircle^1$ & & & & \ding{172}& 5& 1\\
Cl-70& & & & & & & & & \ding{108} & & & & & & & 1& 1\\
Cl-73& & & & & & & & & & & \ding{202} & & & & & 1&1 \\
Cl-76& & & & & & (\ding{173}) & & & & & & & & & & 1&0 \\
Cl-80& & & & & & (\ding{174})& & & & (\ding{172}) & & & (\ding{109}) & & & 3&0 \\
Cl-85& & & & & & & & & & & & (\ding{109})& & & (\ding{202})& 2&1 \\
Cl-86& & & & & & & & & \ding{108} & & & & & & & 1& 1\\
Cl-92& & & & & & & & & & & & & \ding{109}& & & 1& 0\\
Cl-93& & & & & & & & & & & & & \ding{109}& & & 1& 0\\
Cl-99& & & & & & (\ding{172}) (\ding{173}) & & & & & & & & & & 2&0 \\
Cl-102& & & &\ding{202} & & & & & & & & & & & & 1&1 \\
Cl-106& & & & & & & & & & & & & (\ding{109})& &(\ding{202}) & 2&1 \\
Cl-109& & & & & & & & & & \ding{172}& & & & & & 1&0 \\
Cl-115& & & & & & \ding{172} \ding{174} & & & & & & & \ding{109}& & \ding{202} & 4 & 1 \\
Cl-125& & & & & & \ding{172} \ding{174} & & & & & & & & & & 2 & 0 \\
Cl-126& & (\ding{172}) (\ding{174})& & & & \ding{172} \ding{174} & & & & & & & \ding{109}& & \ding{202} & 6 & 1 \\
\hline
L-6 & & & & \ding{175} & & & & & & & & &\ding{108} & & & 2& 1\\
L-7 & & & & & & \ding{172} \ding{174}& & & \ding{109} & \ding{175}& & & \ding{109} & &\ding{202} & 6& 1\\
L-10 & & & & & & $\LEFTcircle^3$ & & & & & & & \ding{109}& & \ding{172}& 3&1 \\
L-12 & & & & & & (\ding{172}) (\ding{174}) & & & & & & & & & & 2&0 \\
L-13 & & & & & & \phantom{x}\hspace{7mm}\phantom{x}& & & & & & & & & \ding{173}& 1& 0\\
L-15 & & & & & & (\ding{172}) (\ding{203}) (\ding{174})& & & & & (\ding{172}) & & & & (\ding{172}) & 5& 1\\
L-18 & & & & & & \ding{174} & & & & & & & & & & 1&0 \\
L-20 & & & & & & (\ding{173})& & & & & & & & & & 1&0 \\
L-21 & & & & & & & & & & & & & \ding{109}& & & 1&0 \\
L-22 & & & & & & \ding{173} \ding{174}& & & & & $\LEFTcircle^1$ & & \ding{109}& & \ding{172} & 5&1 \\
 \hline
\end{tabular}
	


==> tables/aprPartPositionP2.tex <==
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\makecell[l]{\bf Bug}   &   \rotatebox[origin=l]{90}{\bf FP1}   &   \rotatebox[origin=l]{90}{\bf FP2}   &   \rotatebox[origin=l]{90}{\bf FP3}   &   \rotatebox[origin=l]{90}{\bf FP4}   &  \rotatebox[origin=l]{90}{\bf FP5}   &   \rotatebox[origin=l]{90}{\bf FP6}   &   \rotatebox[origin=l]{90}{\bf FP7}   &   \rotatebox[origin=l]{90}{\bf FP8}   &   \rotatebox[origin=l]{90}{\bf FP9}   &   \rotatebox[origin=l]{90}{\bf FP10}   &   \rotatebox[origin=l]{90}{\bf FP11}   &   \rotatebox[origin=l]{90}{\bf FP12}   &   \rotatebox[origin=l]{90}{\bf FP13}   &   \rotatebox[origin=l]{90}{\bf FP14}   &   \rotatebox[origin=l]{90}{F\bf P15}                     &   \rotatebox[origin=l]{90}{\bf \# PP\_FP}                     &   \rotatebox[origin=l]{90}{\bf \# CP\_FP}\\
%\rotatebox[origin=l]{0}{Bug ID} & {\bf FP1} & {\bf FP2} & {\bf FP3} & {\bf FP4}   &  {\bf FP5} & {\bf FP6} & {\bf FP7} & {\bf FP8} & {\bf FP9} & {\bf FP10} & {\bf FP11} & {\bf FP12} & {\bf FP13} & {\bf FP14} & {\bf FP15}                   & {\bf \#-1} & {\bf \#-2}\\
\hline  
L-27 & & & & & & & & & & \ding{173} & & & \ding{109} & & & 2&0 \\
L-30 & & & & (\ding{175}) & & & & & & & & & & & & 1&0 \\
L-33 &&\ding{204}&&&&&&&&&&&&&&1&1 \\
L-39 &&\ding{204}&&\ding{175}&&&&&&&&&\ding{109}&&&3&1 \\
L-47 &&(\ding{203})&&&&&&&&&&&&&&1&1 \\
L-50 &&&&&&&&&&&&&(\ding{109})&&&1&0 \\
L-57 &&\ding{172} \ding{174}&&&&&&&&&&(\ding{109})&\ding{109}&&&4&0 \\
L-58 &&&&&&\ding{172} \ding{174}&&&&&\ding{172}&&&&&3&0 \\
L-59 &&&&&&&&&&&&&\ding{108}&&&1&1 \\
L-63 &&&&&&\ding{174}&&&&\ding{173}&&&\ding{109}&\ding{109}&\ding{172}&5&0 \\
\hline
M-1 &&&&(\ding{175})&&&&&&&&&&&(\ding{172})&2& 0\\
M-3 &&&&&&&&&&&&&\ding{109}&&&1&0 \\
M-4 &&(\ding{202}) (\ding{173})&&&&&&&&&&&&&&2&1 \\
M-5 &&&&&&&&&&&&&\LEFTcircle&&&1&1 \\
M-8 &&&&&&&&&\ding{109}&&&&&&&1&0 \\
M-11 &&&&&&&&\ding{202} \ding{203} \ding{204}&\ding{108}&&&&&&&4&4 \\
M-15 &&&&&&$\LEFTcircle^3$&&&&&&&&&&1&1 \\
M-21 &&&&&&&&&&&&&(\ding{109})&&&1&0 \\
M-22 &&&&&&&&&(\LEFTcircle)&&&&&&&1&1 \\
M-28 &&&&\ding{175}&&\ding{172} \ding{174}&&&\ding{109}&&\ding{172}&&\ding{109}&&\ding{172}&7&0 \\
M-30 &&&&&&&\LEFTcircle &&&&&&&&&1&1 \\
M-32 &&&&&&&&&&&&&&&\ding{172}&1&0 \\
M-33 &&&&\ding{175}&&\ding{174}&&&\ding{109}&&&&\ding{109}&&&4&0 \\
M-35 &&&&(\ding{202})&&&&&&&&&&&&1&1 \\
M-43 &&&&&&(\ding{174})&&&&&&&(\ding{109})&&(\ding{172})&3&0 \\
M-50 &&&&\ding{172} \ding{175}&&\ding{172} \ding{174}&&&\ding{109}&&\ding{172}&&\ding{109}&&$\LEFTcircle^1$&8&1 \\
M-52 &&&&&&\ding{174}&&&&&\ding{172}&&&&&2&0 \\
M-56 &&&&&&&&&&&&&\ding{109}&&&1&0 \\
M-57 &&&&&&&\ding{202}&&&&&&&&&1&1 \\
M-59 &&&&&&&&&&&&&$\LEFTcircle$&&&1&1 \\
M-62 &&&&&&&&&&&&&$\LEFTcircle$&&&1&1 \\
M-63 &&&&&&&&&&&&&$\LEFTcircle$&&&1&1 \\
M-73 &&&&&&&&&&\ding{174}&&&$\LEFTcircle$&&&2&1 \\
M-75 &&&&&&&&&&\ding{202}&&&&&&1&1 \\
M-76 &&(\ding{172}) (\ding{174})&&(\ding{175})&&&&(\ding{172}) (\ding{173})&(\ding{109})&&(\ding{172}) (\ding{175})&&(\ding{109})&(\ding{109})&&10&0 \\
M-77 &&&&(\ding{175})&&&&&&&{\ding{202}}&&(\ding{109})&&(\ding{202})&4& 2\\
M-79 &&&&&&&$\LEFTcircle^1$&&&&&&&&&1&1 \\
M-80 &&&&&&&&&\ding{109}&&\ding{205}&&\ding{109}&&&3&1 \\
M-82 &&&&\ding{175}&&\ding{174}&&&\ding{109}&&\ding{202}&&\ding{109}&&&5&1 \\
M-85 &&&&\ding{109}&&$\LEFTcircle^{1,3}$&&&\ding{109}&&\ding{202}&&\ding{109}&&\ding{172}&7&3 \\
M-86 &&&&&&&&&&&&&(\ding{109})&&&1&0 \\
M-88 &&&&\ding{175}&&\ding{174}&&&&&&&\ding{109}&&&3&0 \\
M-89 & \ding{108} & & & & & & & & & & & & & & & 1&1 \\
M-94 &&&&&&&&&&&&&\ding{109}&&&1&0 \\
M-96 &&&&&&&&&&&\ding{172}&&&&&1&0 \\
M-97 &&&&&&\ding{174}&&&\ding{109}&&&&&&&2&0 \\
M-98 &&&&&&&&&&&&&(\ding{108})&&&1&1 \\
M-99 &&&&&&&&&&&&&(\ding{109})&&&1&0 \\
M-101 &&&&&&&&&&\ding{174}&&&&&&1&0 \\
\hline
Mc-26 & & & & & & & & & \ding{108} & & & & & & & 1 & 1\\
Mc-29 & & \ding{172} \ding{204} & & & & & & & & & & & & & & 2 & 1\\
Mc-38 & & \ding{202} \ding{203} & & & & & & & & & & & & & & 2 & 2\\
\hline
T-2 & & & & \ding{172} & & & & & & & & & & & & 1 & 0\\
T-3 & & & & (\ding{175}) & & & & & & & & & & & & 1 & 0\\
T-7 & & & & & & & & & & & & & \LEFTcircle & & & 1 & 1\\
T-17 & & & & & & & & & \ding{109} & & & & \ding{109} & & & 2 & 0\\
T-18 & & & & & & & & & & & & & & & \ding{173} & 1 & 0\\
T-19 & & & & & & \ding{174} & \ding{202} & & & & & & & & & 2 & 1\\
T-26 & & & & & & & & & & \ding{205} & & & & & & 1 & 1\\
\hline
\hline
Total & 1/1 & 28/16 & 0/0 & 21/3& 0/0& 63/8& 4/4& 5/3& 18/6& 11/4& 25/13& 2/0& 51/13& 4/1& 30/11& 264 &83 \\
\hline
\end{tabular}
	


==> tables/exp2_results_details.tex <==
%\begin{table*}[!h]
%	\centering
%	\scriptsize
%	\caption{Defects4j bugs fixed by \toolname.}
%	\resizebox{1.0\linewidth}{!} {
%	\begin{threeparttable}
%		\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c||c}
%			\toprule
%			FP & 1 & 2.1 & 2.2 & 2.3 & 2.4 & 2.5 & 3& 4.1 & 4.2 & 4.3 & 4.4 & 5& 6.1 & 6.2 & 6.3 & 7.1 & 7.2 & 8.1 & 8.2 & 8.3 & 9.1 & 9.2 & 10.1 & 10.2 & 10.3 & 10.4 & 11.1 & 11.2 & 11.3 & 12 & 13.1 & 13.2 & 14& 15.1 & 15.2 & \\
%
%\hline
%\hline
%\bottomrule
%		\end{tabular}
%	\end{threeparttable}	
%	}
%\end{table*}
%


==> tables/fpVSapr.tex <==
\begin{table}[!h]
	\centering
	\scriptsize
	\caption{Fix Pattern Qualitative.}
%	\resizebox{1\linewidth}{!}{
	\begin{threeparttable}
		\begin{tabular}{l|c|c}
			\toprule
			{\bf APR Tool} & {\bf \# of fix patterns} & {\bf \# fixed Bugs} \\
			\hline
			\rowcolor{lightgray}
			jMutRepair & 1  & 3/17\\
			ssFix      & 9  & 20/60\\
			\rowcolor{lightgray}
			ELIXIR     & 12 & 26/41\\
			PAR        & 13 & 18/49$^\ast$\\
			\rowcolor{lightgray}
			FixMiner   & 13 & 25/31\\
			AVATAR     & 14 & 30/61\\
			\rowcolor{lightgray}
			SketchFix  & 15 & 19/26\\
			SOFix      & 16 & -/23\\	
			\rowcolor{lightgray}
			HDRepair   &	 16 & 6/23\\	
%			S3         & 6  &\\
%			NPEfix     & 4 & \\
			CapGen     & 18 & 21/25\\
			\rowcolor{lightgray}
			SimFix     & 19 & 34/56\\
			\bottomrule
		\end{tabular}
	\end{threeparttable}
%	}
	\label{tab:fpVSapr}
\end{table}

==> tables/statisticFixBugs.tex <==
\begin{table}[!h]
	\centering
	\scriptsize
	\caption{Statistics of Fixed Bugs.}
%	\resizebox{1\linewidth}{!}{
	\begin{threeparttable}
		\begin{tabular}{l|c|c}
			\toprule
			 & Plausibly fixed & Correctly fixed\\
			\hline
			\# of bugs fixed by single fix patterns & 65 & 37\\
			\# of bugs fixed by several fix patterns & 55 & 43(33)\\
			\bottomrule
		\end{tabular}
	\end{threeparttable}
%	}
	\label{tab:statFB}
\end{table}
